PhysHanDI: Physics-Based Reconstruction of Hand-Deformable Object Interactions

While existing methods for reconstructing hand-object interactions have made impressive progress, they either focus on rigid or part-wise rigid objects-limiting their ability to model real-world objects (e.g., cloth, stuffed animals) that exhibit highly non-rigid deformations-or model deformable objects without full 3D hand reconstruction. To bridge this gap, we present PhysHanDI (Physics-based Reconstruction of Hand and Deformable Object Interactions), a framework that enables full 3D reconstruction of both interacting hands and non-rigid objects. Our key idea is to physically simulate object deformations driven by forces induced from densely reconstructed 3D hand motions, ensuring that the reconstructed object dynamics are both physically plausible and coherent with the interacting hand movements. Furthermore, we demonstrate that such simulation of object deformations can, in turn, refine and improve hand reconstruction via inverse physics. In experiments, PhysHanDI outperforms the state-of-the-art baseline across reconstruction and future prediction.

==> tab/hyperparam_manual.tex <==
\begin{table}[!h]
\centering
\small
\begin{tabular}{clccccc}
\toprule
\textbf{Row} & \textbf{Method} & \textbf{$\delta$ Setting} & \textbf{$\delta$} & $\text{CD}_\text{full}$ $\downarrow$ & \textbf{PSNR} $\uparrow$ \\
\midrule
A & PhysTwin~\cite{jiang2025phystwin}                & Optimized          & 0.0331 & 8.86          & 22.48 \\
B & \textbf{\textsc{PhysHanDI} (Ours)}                & Optimized          & 0.0306 & \textbf{4.44} & \textbf{24.60} \\
\midrule
C & \textsc{PhysHanDI} (Ours)                        & Manually assigned  & 0.002  & 24.89         & 19.46 \\
D & \textsc{PhysHanDI} (Ours)                        & Manually assigned  & 0.02   & \textbf{4.44}          & \underline{24.42} \\
E & \textsc{PhysHanDI} (Ours)                        & Manually assigned  & 0.04   & \underline{4.49}          & 24.36 \\
\bottomrule
\end{tabular}
\vspace{0.5\baselineskip}
\caption{\textbf{Effect of bypassing the zero-order optimization with a manually assigned $\delta$} on the \texttt{double\_stretch\_sloth} sequence (Reconstruction \& Resimulation, multi-view RGB-D inputs). Rows A--B use the optimized $\delta$; rows C--E replace the optimized $\delta$ in our method with manually assigned values. Performance is robust to moderate manual values (rows D, E), but a too-small $\delta$ (row C) removes critical contact connections and causes catastrophic degradation.}
\label{tab:hyperparam_manual}
\vspace{-0.5\baselineskip}
\end{table}


==> tab/morebaselines_gsdynamics.tex <==
\begin{table}[!h]
\centering
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|cc|cccc|cc|cccc}
\toprule
\multirow{3}{*}{\textbf{Method}} & \multicolumn{6}{c|}{\textbf{Reconstruction \& Resimulation}} & \multicolumn{6}{c}{\textbf{Future Prediction}} \\
\cmidrule(lr){2-13}
\multirow{2}{*}{} & \multicolumn{2}{c|}{\textbf{3D Metrics}} & \multicolumn{4}{c|}{\textbf{2D Metrics}} & \multicolumn{2}{c|}{\textbf{3D Metrics}} & \multicolumn{4}{c}{\textbf{2D Metrics}} \\
 & CD $\downarrow$ & Track Err. $\downarrow$ & IoU \% $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & CD $\downarrow$ & Track Err. $\downarrow$ & IoU \% $\uparrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
\midrule
\multicolumn{13}{c}{\textbf{(a) Results on the dense interaction sequences.}} \\
\midrule
Spring-Gaus~\cite{zhong2024reconstruction} & 38.84&	4.65&	0.55&	21.41&	0.94&	7.80&	56.51&	7.69&	0.42&	19.91&	\textbf{0.94} & 9.27 \\
GS-Dynamics~\cite{zhang2024dynamics} & 13.67& 1.81& 0.74& 23.12& 0.94& 3.80& 33.99& 4.50& 0.51& 18.97& 0.93& 7.79\\
PhysTwin~\cite{jiang2025phystwin} & 5.90&	1.00&	0.84&	25.23&	\textbf{0.95}&	2.65&	11.45&	2.10&	0.70&	22.07&	\textbf{0.94}&	5.38 \\
\textbf{\textsc{PhysHanDI} (Ours)} & \textbf{5.30}&	\textbf{0.89}& \
\textbf{0.85}&	\textbf{25.62}&	\textbf{0.95}&	\textbf{2.52}&	\textbf{10.57}&	\textbf{2.05}&	\textbf{0.73}&	\textbf{22.84}&	\textbf{0.94}&	\textbf{4.83}\\
\midrule
\multicolumn{13}{c}{\textbf{(b) Results on the full sequences.}} \\
\midrule
Spring-Gaus~\cite{zhong2024reconstruction} & 33.60&	4.07&	0.62&	21.24&	0.94&	8.09&	46.54&	6.61 &	0.48&	19.59&	0.93 & 9.44 \\
GS-Dynamics~\cite{zhang2024dynamics} & 13.79& 2.18& 0.72& 24.01& \textbf{0.95}& 4.14& 38.84& 6.88& 0.46& 19.38& 0.94& 8.32\\
PhysTwin~\cite{jiang2025phystwin} & 5.52&	0.97&	\textbf{0.84}&	26.32&	\textbf{0.95}&	2.88&	12.26&	2.44&	\textbf{0.69}&	22.80&	\textbf{0.95}&	5.15 \\
\textbf{\textsc{PhysHanDI} (Ours)} & \textbf{5.40}&	\textbf{0.96}& \textbf{0.84}&	\textbf{26.44}&	\textbf{0.95}&	\textbf{2.87}&	\textbf{12.04}&	\textbf{2.41}&	0.68&	\textbf{22.96}&	\textbf{0.95}&	\textbf{5.02}\\

\bottomrule
\end{tabular}
}
\caption{\textbf{Reconstruction \& Resimulation and Future Prediction results on the PhysTwin dataset~\citep{jiang2025phystwin}}. $\textrm{CD}$ is measured in millimeters, and $\textrm{Track Err.}$ and $\textrm{LPIPS}$ are scaled by $\times100$ for readability.}
\label{tab:morebaselines_gsdynamics}
\end{table}


